A Study on the Autoregressive and non-Autoregressive Multi-label Learning

Extreme classification tasks are multi-label tasks with an extremely large number of labels (tags). These tasks are hard because the label space is usually (i) very large, e.g. thousands or millions of labels, (ii) very sparse, i.e. very few labels apply to each input document, and (iii) highly correlated, meaning that the existence of one label changes the likelihood of predicting all other labels. In this work, we propose a self-attention based variational encoder-model to extract the label-label and label-feature dependencies jointly and to predict labels for a given input. In more detail, we propose a non-autoregressive latent variable model and compare it to a strong autoregressive baseline that predicts a label based on all previously generated labels. Our model can therefore be used to predict all labels in parallel while still including both label-label and label-feature dependencies through latent variables, and compares favourably to the autoregressive baseline. We apply our models to four standard extreme classification natural language data sets, and one news videos dataset for automated label detection from a lexicon of semantic concepts. Experimental results show that although the autoregressive models, where use a given order of the labels for chain-order label prediction, work great for the small scale labels or the prediction of the highly ranked label, but our non-autoregressive model surpasses them by around 2% to 6% when we need to predict more labels, or the dataset has a larger number of the labels.

==> VAE_ML 2/ensemble_table_nDCG.tex <==
\begin{table}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lcccc }
\toprule
&& \textbf{Proposed} & \textbf{SLEEC} &	\textbf{FastXML}	 \\
\midrule
\multirow{3}{*}{\textbf{Bibtex}} & 
nDCG@1	 & \textit{64.56} & \textbf{65.08} & 63.42 \\ &
nDCG@3   & \textit{60.11} & \textbf{60.47} & 59.51 \\ &
nDCG@5	 & \textit{62.18} & \textbf{62.64} & 61.70 \\ 
\midrule
\multirow{3}{*}{\textbf{Delicious}} & 
nDCG@1	& 65.13 & 67.59 & \textbf{69.61}\\ &
nDCG@3	& 60.51 & 62.87 & \textbf{65.47}\\ &
nDCG@5	& 57.12 & 59.28 & \textbf{61.90} \\ 
\midrule
\multirow{3}{*}{\textbf{Mediamill}} & 
nDCG@1	 &  84.25 & \textbf{87.82} & 84.22 \\ &
nDCG@3	 &  75.33 & \textbf{81.50} & 75.41 \\ &
nDCG@5	 &  72.03 & \textbf{79.22} & 72.37 \\ 
\midrule
\multirow{3}{*}{\textbf{Eurlex}} & 
nDCG@1	 & \textbf{81.04} & 79.26 & 71.36 \\ &
nDCG@3	 & \textbf{71.29} & 68.13 & 62.87 \\ &
nDCG@5	 & \textbf{65.64} & 61.60 & 58.06 \\ 
\midrule
\multirow{3}{*}{\textbf{Wiki10}} & 
nDCG@1	& \textbf{86.05} & 85.88 & 84.31 \\ &
nDCG@3	& \textbf{79.11} & 72.98 & 75.35 \\ &
nDCG@5	& \textbf{72.26} & 62.70 & 63.36 \\  
\bottomrule
\end{tabular} \caption{nDCG@k on the ensemble-based nonlinear models. Best in \textbf{bold} and not significantly different to best in \textit{italics}.}\label{tbl_ensemble_d1}

\end{table} 

==> VAE_ML 2/ensemble_table_p.tex <==
\begin{table}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lcccc }
\toprule
&& \textbf{Proposed} & \textbf{SLEEC} &	\textbf{FastXML}	 \\
\midrule
\multirow{3}{*}{\textbf{Bibtex}} & P@1 & \textit{64.56}$\pm$0.79 & \textbf{65.08}$\pm$0.65 &  63.42$\pm$0.67\\
& P@3 & \textit{39.51}$\pm$0.34 & \textbf{39.64}$\pm$0.39 &  39.23$\pm$0.57\\
& P@5 & \textit{28.80}$\pm$0.26 & \textbf{28.87}$\pm$0.32&  28.86$\pm$0.38\\

\midrule
\multirow{3}{*}{\textbf{Delicious}} & P@1 & 65.13$\pm$0.39 & 67.59$\pm$0.53 & \textbf{69.61}$\pm$0.58 \\
& P@3 & 59.07$\pm$0.41 & 61.38$\pm$0.59 & \textbf{64.12}$\pm$0.75 \\
& P@5	& 54.52$\pm$0.34 & 56.56$\pm$0.54 & \textbf{59.27}$\pm$0.65 \\

\midrule
\multirow{3}{*}{\textbf{Mediamill}} & P@1	& 84.25$\pm$0.27 & \textbf{87.82}$\pm$0.33 & 84.22$\pm$0.27 \\
& P@3	& 67.29$\pm$0.24 & \textbf{73.45}$\pm$0.30 & 67.33$\pm$0.20 \\
& P@5	& 52.90$\pm$0.15 & \textbf{59.17}$\pm$0.34 & 53.04$\pm$0.18 \\

\midrule
\multirow{3}{*}{\textbf{Eurlex}} & P@1	& \textbf{81.04}$\pm$0.81 & 79.26$\pm$0.86 & 71.36$\pm$1.63 \\
& P@3	& \textbf{67.91}$\pm$0.97 & 64.30$\pm$0.88 & 59.90$\pm$1.58 \\
& P@5	& \textbf{56.81}$\pm$0.97 & 52.33$\pm$0.80 & 50.39$\pm$1.40 \\

\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} & P@1	& \textbf{86.05} & 85.88 &  83.03\\
& P@3	& \textbf{76.85} & 72.98 &  67.47\\
& P@5	& \textbf{67.77} & 62.70 &  57.76\\
\bottomrule
\end{tabular}  \caption{Validation precision@k for ensemble-based non-linear models. Best in \textbf{bold} and not significantly different to best in \textit{italics}.}\label{tbl_ensemble_p1} 

\end{table}

==> VAE_ML 2/modified_table_1.tex <==
\begingroup
\setlength{\tabcolsep}{5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.0} % Default
\begin{table*}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lccccccc cccccc }
\toprule
&& \multicolumn{2}{c}{\textbf{Proposed}} & \multicolumn{2}{c}{\textbf{PD-sparse}} &	\multicolumn{2}{c}{\textbf{LEML}} &	\multicolumn{2}{c}{\textbf{CPLST}} &	\multicolumn{2}{c}{\textbf{CS}} &	\multicolumn{2}{c}{\textbf{ML-CSSP}} \\
\midrule
&  & \textbf{P} & \textbf{nDCG} & \textbf{P} & \textbf{nDCG} &	\textbf{P} & \textbf{nDCG} &	\textbf{P} & \textbf{nDCG} &	\textbf{P} & \textbf{nDCG} &	\textbf{P} & \textbf{nDCG} \\
\midrule
\multirow{3}{*}{\textbf{Bibtex}} & \textbf{@1}	&  \textbf{64.56}  & \red{00.0} & 61.29  & \red{00.0} & 62.54 & \red{00.0} & 62.38 & \red{00.0} & 58.87 & \red{00.0} & 44.98 &  \red{00.0}  \\
& \textbf{@3} &  \textbf{39.51}  & \red{00.0} & 35.82  & \red{00.0} & 38.41 & \red{00.0} & 37.84 & \red{00.0} & 33.53 & \red{00.0} & 30.43 &  \red{00.0}  \\
& \textbf{@5}	& \textbf{28.80}  & \red{00.0} & 25.74 & \red{00.0} & 28.21 & \red{00.0} & 27.62 & \red{00.0} & 23.72 & \red{00.0} & 23.53 &  \red{00.0}    \\
%\midrule
%\multicolumn{7}{c}{Delicious}	\\
\midrule
\multirow{3}{*}{\textbf{Delicious}} & \textbf{@1}	& \textbf{65.13} & \red{00.0} & 51.82  & \red{00.0} & \textbf{65.67} & \red{00.0} & \textbf{65.31} & \red{00.0} & 61.36 & \red{00.0} & 63.04 &  \red{00.0}  \\
& \textbf{@3}	&  59.07 & \red{00.0} & 44.18  & \red{00.0} & \textbf{60.55} & \red{00.0} & 59.95 & \red{00.0} & 56.46 & \red{00.0} & 56.26 &  \red{00.0}  \\
& \textbf{@5}	& 54.52 & \red{00.0} & 38.95  & \red{00.0} & \textbf{56.08} & \red{00.0} & 55.31 & \red{00.0} & 52.07 & \red{00.0} & 50.16 & \red{00.0}   \\
\midrule
\multirow{3}{*}{\textbf{Mediamill}} & \textbf{@1}	& \textbf{84.25} & \red{00.0} & 81.86  & \red{00.0} & \textbf{84.01} & \red{00.0} & 83.35 & \red{00.0} & \textbf{83.82} & \red{00.0} & 78.95 &  \red{00.0}  \\
& \textbf{@3}	&  \textbf{67.29} & \red{00.0} & 62.52  & \red{00.0} & \textbf{67.20} & \red{00.0} & 66.18 & \red{00.0} & \textbf{67.32} & \red{00.0} & 60.93 &  \red{00.0}  \\
& \textbf{@5}	 & \textbf{52.90} & \red{00.0}  & 45.11 & \red{00.0} & 52.80 & \red{00.0} & 51.46 & \red{00.0} & 52.80 & \red{00.0} & 44.27 &  \red{00.0}  \\
%\midrule
%\multicolumn{7}{c}{Eurlex} \\
\midrule
\multirow{3}{*}{\textbf{Eurlex}}  & \textbf{@1}	& \textbf{81.04} & \red{00.0} & 76.43  & \red{00.0} & 63.40 & \red{00.0} & 72.28 & \red{00.0} & 58.52 & \red{00.0} & 62.09 &  \red{00.0}  \\
& \textbf{@3}	& \textbf{67.91} & \red{00.0} & 60.37 & \red{00.0} & 50.35 & \red{00.0} & 58.16 & \red{00.0} & 45.51 & \red{00.0} & 48.39 &  \red{00.0}  \\
& \textbf{@5}	& \textbf{56.81} & \red{00.0} & 49.72 & \red{00.0} & 41.28 & \red{00.0} & 47.73 & \red{00.0} & 32.47 & \red{00.0} & 40.11 & \red{00.0}  \\
%\midrule
%\multicolumn{7}{c}{Wiki10-31k}	\\
\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} & \textbf{@1}	& \textbf{86.05} & \red{00.0} & 82.14 & \red{00.0} & 73.47 & \red{00.0} & -- & -- & -- & -- & -- &  -- \\
& \textbf{@3}	& \textbf{76.85} & \red{00.0} & 69.68 & \red{00.0} & 62.43 & \red{00.0} & -- & -- & -- & -- & -- & --  \\
& \textbf{@5}	& \textbf{67.77} & \red{00.0} & 58.76 & \red{00.0} & 54.35 & \red{00.0} & -- & -- & -- & -- & -- &  -- \\
\bottomrule
\end{tabular} \caption{Validation set top-$k$ label precision (P@k) and normalised Discounted Cumulative Gain (nDCG@k). We show means over 10 runs with single models and $k=100$ or $30$ (Mediamill). Best model(s) per metric highlighted in \textbf{bold} ($p=0.05$). In supplementary material we additionally report all models' variances.}\label{tbl_smallp1_m}
\end{table*} 
\endgroup

==> VAE_ML 2/original_table_nDCG.tex <==

\begin{table*}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lccccccccccc }
\toprule
&& \textbf{Seq2Seq} & \textbf{nAR} & \textbf{SLEEC} &	\textbf{FastXML} & \textbf{PD-sparse} &	\textbf{LEML} &	\textbf{CPLST} &	\textbf{CS} &	\textbf{ML-CSSP} \\
\midrule

\multirow{3}{*}{\textbf{Bibtex}} & 
nDCG@1	 & \textbf{93.57}$\pm$0.73 & 49.94$\pm$1.33 &  65.08 & 63.42 & 61.29$\pm$0.65  & 62.54$\pm$0.52 & 62.38$\pm$0.63 & 58.87$\pm$0.61 & 44.98$\pm$1.15  \\ 
& nDCG@3   & \textbf{71.58}$\pm$1.28 & 28.49$\pm$1.21 & 60.47 & 59.51 & 55.83$\pm$0.57  & 58.22$\pm$0.42 & 57.63$\pm$0.56 & 52.19$\pm$0.56 & 44.67$\pm$1.01 \\ 
& nDCG@5	 & \textbf{69.12}$\pm$1.22 & 20.67$\pm$1.51& 62.64 & 61.70 & 57.35$\pm$0.49  & 60.53$\pm$0.38 & 59.71$\pm$0.42 & 53.25$\pm$0.54 & 47.97$\pm$0.98  \\ 
\midrule
\multirow{3}{*}{\textbf{Delicious}} & 
nDCG@1	&\textbf{97.36}$\pm$0.37 & 61.78$\pm$0.91& 67.59 & 69.61& 51.82$\pm$1.40  & 65.67$\pm$0.73 & 65.31$\pm$0.88 & 61.36$\pm$0.38 & 63.04$\pm$1.29  \\ 
& nDCG@3	& \textbf{76.23}$\pm$0.69 & 57.56$\pm$0.83& 62.87 & 65.47& 46.00$\pm$1.12  & 61.77$\pm$0.50 & 61.16$\pm$0.45 & 57.66$\pm$0.34 & 57.91$\pm$1.15 \\
& nDCG@5	&57.73$\pm$0.71 & 53.98$\pm$0.82& 59.28 & \textbf{61.90}& 42.02$\pm$1.01  & 58.47$\pm$0.47 & 57.80$\pm$0.49 & 54.44$\pm$0.32 & 53.36$\pm$0.94  \\ 
\midrule
\multirow{3}{*}{\textbf{Mediamill}} &
nDCG@1	 &\textbf{93.57}$\pm$0.35 & 77.14$\pm$0.21&87.82 & 84.22 &  81.86$\pm$4.08  & 84.01$\pm$0.31 & 83.35$\pm$0.33 & 83.82$\pm$5.92 & 78.95$\pm$0.23 	 \\ 
& nDCG@3	 & \textbf{82.81}$\pm$0.79 & 58.64$\pm$0.69& 81.50 & 75.41 &  70.21$\pm$2.37  & 75.23$\pm$0.25 & 74.21$\pm$0.24 & 75.29$\pm$4.99 & 68.97$\pm$0.28  \\ 
& nDCG@5	 &  71.88$\pm$0.75 & 46.12$\pm$0.23 &\textbf{79.22} & 72.37 &  63.71$\pm$1.73  & 71.96$\pm$0.18 & 70.55$\pm$0.17 & 71.92$\pm$4.03 & 62.88$\pm$0.26  \\ 
\midrule
\multirow{3}{*}{\textbf{Eurlex}} &
nDCG@1	 & \textbf{83.18}$\pm$0.97 & 54.92$\pm$6.06&79.26 & 71.36 &  76.43$\pm$1.04  & 63.40$\pm$1.58 & 72.28$\pm$0.99 & 58.52$\pm$1.06 & 62.09$\pm$2.12  \\ 
& nDCG@3	 & 55.61$\pm$2.32 & 44.69$\pm$5.14& \textbf{68.13} & 62.87  &  64.31$\pm$0.72  & 53.56$\pm$1.47 & 61.64$\pm$1.02 & 48.67$\pm$0.75 & 51.63$\pm$1.31  \\ 
& nDCG@5	 & 42.67$\pm$1.86 & 40.06$\pm$4.75&\textbf{61.60} & 58.06 &  58.78$\pm$0.70  & 48.47$\pm$1.24 & 55.92$\pm$0.97 & 40.79$\pm$0.65 & 47.11$\pm$1.10  \\ 
\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} &
nDCG@1	&  74.16$\pm$2.37 & 76.03& \textbf{85.88} & 84.31 & 82.14  & 73.47 & - & - & -   \\ 
& nDCG@3	& 37.56$\pm$0.36 & 67.22& 72.98 & \textbf{75.35}  & 72.63  & 64.92 & - & - & -   \\ 
& nDCG@5	& 27.17$\pm$0.25 & 61.00& 62.70 & 63.36 & \textbf{64.33}  & 58.69 & - & - & -   \\
\bottomrule
\end{tabular} \caption{nDCG@k on the small-scale datasets. Best in \textbf{bold}.}\label{tbl_smalld1}
\end{table*} 

==> VAE_ML 2/original_table_precisions.tex <==
\begin{table*}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lccccccccccc }
\toprule
&& \textbf{Seq2Seq} & \textbf{nAR} & \textbf{SLEEC} &	\textbf{FastXML} & \textbf{PD-sparse} &	\textbf{LEML} &	\textbf{CPLST} &	\textbf{CS} &	\textbf{ML-CSSP} \\
\midrule

\multirow{3}{*}{\textbf{Bibtex}} & P@1	&  \textbf{93.57}$\pm$0.73 & 49.92$\pm$1.3 & 65.08$\pm$0.65 &  63.42$\pm$0.67 &  61.29$\pm$0.65  & 62.54$\pm$0.52 & 62.38$\pm$0.63 & 58.87$\pm$0.61 & 44.98$\pm$1.15   \\
& P@3 & 36.65$\pm$0.95 & 28.49$\pm$0.73 & \textbf{39.64}$\pm$0.39 &  39.23$\pm$0.57 & 35.82$\pm$0.46  & 38.41$\pm$0.42 & 37.84$\pm$0.48 & 33.53$\pm$0.49 & 30.43$\pm$0.59   \\
& P@5	& 21.99$\pm$0.57 & 20.67$\pm$0.67 & \textbf{28.87}$\pm$0.32&  28.86$\pm$0.38  & 25.74$\pm$0.30 & 28.21$\pm$0.24 & 27.62$\pm$0.27 & 23.72$\pm$0.29 & 23.53$\pm$0.37     \\
\midrule
\multirow{3}{*}{\textbf{Delicious}} & P@1	& \textbf{97.36}$\pm$0.37 & 61.78$\pm$0.91 & 67.59$\pm$0.53 & 69.61$\pm$0.58 & 51.82$\pm$1.40  & 65.67$\pm$0.73 & 65.31$\pm$0.88 & 61.36$\pm$0.38 & 63.04$\pm$1.28  \\
& P@3	& \textbf{69.40}$\pm$0.98 & 56.24$\pm$0.84 & 61.38$\pm$0.59 & 64.12$\pm$0.75  & 44.18$\pm$1.04  & 60.55$\pm$0.48 & 59.95$\pm$0.43 & 56.46$\pm$0.33 & 56.26$\pm$1.13 \\
& P@5	& 45.07$\pm$0.93 & 51.46$\pm$0.84 & 56.56$\pm$0.54 & \textbf{59.27}$\pm$0.65 & 38.95$\pm$0.94  & 56.08$\pm$0.43 & 55.31$\pm$0.50 & 52.07$\pm$0.30 & 50.16$\pm$0.83  \\
\midrule
\multirow{3}{*}{\textbf{Mediamill}} & P@1	& \textbf{93.57}$\pm$0.35 & 77.14$\pm$0.21 & 87.82$\pm$0.33 & 84.22$\pm$0.27 & 81.86$\pm$4.08  & 84.01$\pm$0.31 & 83.35$\pm$0.33 & 83.82$\pm$5.92 & 78.95$\pm$0.23  \\
& P@3	& 71.81$\pm$1.23 & 58.64$\pm$0.32 & \textbf{73.45}$\pm$0.30 & 67.33$\pm$0.20& 62.52$\pm$2.31  & 67.20$\pm$0.23 & 66.18$\pm$0.22 & 67.32$\pm$4.42 & 60.93$\pm$0.24  \\
& P@5	 & 46.55$\pm$0.97 & 46.12$\pm$0.11 &  \textbf{59.17}$\pm$0.34 & 53.04$\pm$0.18 & 45.11$\pm$1.14 & 52.80$\pm$0.18 & 51.46$\pm$0.20 & 52.80$\pm$2.61 & 44.27$\pm$0.20  \\
\midrule
\multirow{3}{*}{\textbf{Eurlex}} & P@1	& \textbf{83.18}$\pm$0.97 & 54.93$\pm$6.06  & 79.26$\pm$0.86 & 71.36$\pm$1.63 & 76.43$\pm$1.04  & 63.40$\pm$1.58 & 72.28$\pm$0.99 & 58.52$\pm$1.06 & 62.09$\pm$2.12 \\
& P@3	& 46.90$\pm$2.89 & 41.50$\pm$4.89 & \textbf{64.30}$\pm$0.88 & 59.90$\pm$1.58 & 60.37$\pm$0.74  & 50.35$\pm$1.44 & 58.16$\pm$1.11 & 45.51$\pm$0.71 & 48.39$\pm$1.31  \\
& P@5	& 28.56$\pm$1.88 & 33.61$\pm$4.14& \textbf{52.33}$\pm$0.80 & 50.39$\pm$1.40 & 49.72$\pm$0.74  & 41.28$\pm$1.07 & 47.73$\pm$0.97 & 32.47$\pm$0.58 & 40.11$\pm$1.10  \\
\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} & P@1	& 74.16$\pm$2.37 & 76.03 & \textbf{85.88} &  83.03 & 82.14 & 73.47 & - & - & - \\
& P@3	& 27.88$\pm$0.29 & 64.63 & \textbf{72.98} &  67.47 & 69.68 & 62.43 & - & - & - \\
& P@5	& 16.75$\pm$0.18 & 56.60 &\textbf{62.70} &  57.76 & 58.76 & 54.35 & - & - & - \\
\bottomrule
\end{tabular} \caption{Validation set precision@k for single models. Best in \textbf{bold}.}\label{tbl_smallp1}
\end{table*} 


==> VAE_ML 2/table_seq2seq_PSndcgs.tex <==

\begin{table}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lccc }
\toprule
&& \textbf{Seq2Seq} & \textbf{nAR} \\
\midrule

\multirow{3}{*}{\textbf{Bibtex}}
& PSnDCG@1	& \textbf{84.41}$\pm$0.69 & 36.42$\pm$1.10 \\
& PSnDCG@3	& \textbf{67.06}$\pm$1.29 & 35.96$\pm$1.15 \\
& PSnDCG@5	& \textbf{65.50}$\pm$1.25 & 38.07$\pm$1.42 \\
\midrule
\multirow{3}{*}{\textbf{Delicious}} 
& PSnDCG@1	& \textbf{62.79}$\pm$0.34 & 23.15$\pm$0.43 \\
& PSnDCG@3	& \textbf{49.93}$\pm$0.36 & 24.48$\pm$0.41 \\
& PSnDCG@5	& \textbf{40.14}$\pm$0.42 & 25.06$\pm$0.44 \\
\midrule
\multirow{3}{*}{\textbf{Mediamill}} 
& PSnDCG@1	& \textbf{86.41}$\pm$0.36 & 55.01$\pm$0.11 \\
& PSnDCG@3	& \textbf{79.15}$\pm$0.72 & 53.47$\pm$0.53 \\
& pSnDCG@5	& \textbf{70.41}$\pm$0.71 & 54.10$\pm$0.15 \\
\midrule
\multirow{3}{*}{\textbf{Eurlex}} 
& PSnDCG@1	& \textbf{34.13}$\pm$0.42 & 27.54$\pm$4.66 \\
& pSnDCG@3	& \textbf{29.47}$\pm$1.51 & 26.35$\pm$4.44 \\
& PSnDCG@5	& 25.74$\pm$1.37 & \textbf{26.42}$\pm$4.65 \\
\midrule
%\multirow{3}{*}{\textbf{Eurlex-4.3K}} 
%& PSnDCG@1	& \textbf{39.89}$\pm$0.24 & --- \\
%& PSnDCG@3	& \textbf{48.17}$\pm$1.31 & --- \\
%& PSnDCG@5	& \textbf{44.48}$\pm$1.65 & --- \\
%\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} 
& PSnDCG@1	& 8.37$\pm$0.25 & \textbf{14.15} \\
& PSnDCG@3	& 4.78$\pm$0.03 & \textbf{13.58} \\
& PSnDCG@5	& 3.83$\pm$0.02 & \textbf{13.49} \\
\bottomrule
\end{tabular} \caption{Single model propensity scored nDCG@k. Showing mean and standard deviations over 10 different publicly-available train/validation splits. Best in \textbf{bold} }\label{tab:baseline_seq2seq_ndcg_with_propensity}
\end{table}


==> VAE_ML 2/table_seq2seq_PSprecisions.tex <==

\begin{table}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lccc }
\toprule
&& \textbf{Seq2Seq} & \textbf{nAR} \\
\midrule

\multirow{3}{*}{\textbf{Bibtex}}
& PSP@1 & \textbf{84.41}$\pm$0.69 & 36.42$\pm$1.10 \\
& PSP@3 & \textbf{51.37}$\pm$1.53 & 36.09$\pm$1.21 \\
& PSP@5 & \textbf{45.36}$\pm$1.33 & 39.78$\pm$1.77 \\
\midrule
\multirow{3}{*}{\textbf{Delicious}} 
& PSP@1	& \textbf{62.79}$\pm$0.34 & 23.15$\pm$0.43 \\
& PSP@3	& \textbf{45.63}$\pm$0.55 & 24.48$\pm$0.42 \\
& PSP@5	& \textbf{32.15}$\pm$0.59 & 25.06$\pm$0.46 \\
\midrule
\multirow{3}{*}{\textbf{Mediamill}} 
& PSP@1	& \textbf{86.41}$\pm$0.36 & 55.01$\pm$0.11 \\
& PSP@3	& \textbf{74.97}$\pm$1.25 & 53.12$\pm$0.23 \\
& PSP@5	& \textbf{59.23}$\pm$1.19 & 52.45$\pm$0.09 \\
\midrule
\multirow{3}{*}{\textbf{Eurlex}} 
& PSP@1	& \textbf{34.13}$\pm$0.42 & 27.54$\pm$4.66 \\
& PSP@3	& \textbf{27.22}$\pm$1.96 & 25.97$\pm$4.37 \\
& PSP@5	& 21.03$\pm$1.61 & \textbf{26.17}$\pm$4.40 \\
\midrule
%\multirow{3}{*}{\textbf{Eurlex-4.3K}} 
%& PSP@1	& 39.89$\pm$0.24 & --- \\
%& PSP@3	& 50.14$\pm$1.94 & --- \\
%& PSP@5	& 41.99$\pm$2.35 & --- \\
%\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} 
& PSP@1	& 8.37$\pm$0.25 & \textbf{14.15} \\
& PSP@3	& 3.69$\pm$0.04 & \textbf{13.42} \\
& PSP@5	& 2.55$\pm$0.03 & \textbf{13.34} \\
\bottomrule
\end{tabular} \caption{Single model propensity scored precision@k. Showing mean and standard deviations over 10 different publicly-available train/validation splits. Best in \textbf{bold}}\label{tab:baseline_seq2seq_precisions_with_propensity}
\end{table}


==> VAE_ML 2/table_seq2seq_ndcgs.tex <==
\begin{table}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lccc }
\toprule
&& \textbf{Seq2Seq} & \textbf{nAR} \\
\midrule

\multirow{3}{*}{\textbf{Bibtex}}
& nDCG@1    & \textbf{93.57}$\pm$0.73 & 49.94$\pm$1.33 \\
& nDCG@3    & \textbf{71.58}$\pm$1.28 & 28.49$\pm$1.21 \\
& nDCG@5    & \textbf{69.12}$\pm$1.22 & 20.67$\pm$1.51 \\
\midrule
\multirow{3}{*}{\textbf{Delicious}} 
& nDCG@1    & \textbf{97.36}$\pm$0.37 & 61.78$\pm$0.91 \\
& nDCG@3    & \textbf{76.23}$\pm$0.69 & 57.56$\pm$0.83 \\
& nDCG@5    & \textbf{57.73}$\pm$0.71 & 53.98$\pm$0.82 \\
\midrule
\multirow{3}{*}{\textbf{Mediamill}} 
& nDCG@1	& \textbf{93.57}$\pm$0.35 & 77.14$\pm$0.21 \\
& nDCG@3	& \textbf{82.81}$\pm$0.79 & 66.05$\pm$0.69 \\
& nDCG@5	& \textbf{71.88}$\pm$0.75 & 63.51$\pm$0.23 \\
\midrule
\multirow{3}{*}{\textbf{Eurlex}} 
& nDCG@1	& \textbf{83.18}$\pm$0.97 & 54.92$\pm$6.06 \\
& nDCG@3	& \textbf{55.61}$\pm$2.32 & 44.69$\pm$5.14 \\
& nDCG@5	& \textbf{42.67}$\pm$1.86 & 40.06$\pm$4.75 \\
\midrule
%\multirow{3}{*}{\textbf{Eurlex-4.3K}} 
%& nDCG@1	& \textbf{85.99}$\pm$0.39 & --- \\
%& nDCG@3	& \textbf{77.37}$\pm$1.61 & --- \\
%& nDCG@5	& \textbf{64.83}$\pm$1.88 & --- \\
%\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} 
& nDCG@1	& 74.16$\pm$2.37 & \textbf{76.03} \\
& nDCG@3	& 37.56$\pm$0.36 & \textbf{67.22} \\
& nDCG@5	& 27.17$\pm$0.25 & \textbf{61.00} \\
\bottomrule
\end{tabular} \caption{Single model nDCG@k. Showing mean and standard deviations over 10 different publicly-available train/validation splits. Best in \textbf{bold}.}\label{tab:baseline_seq2seq_ndcg_no_propensity}
\end{table}


==> VAE_ML 2/table_seq2seq_precisions.tex <==
\begin{table}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lccc }
\toprule
&& \textbf{Seq2Seq} & \textbf{nAR} \\
\midrule

\multirow{3}{*}{\textbf{Bibtex}}
& P@1 & \textbf{93.57}$\pm$0.73 & 49.92$\pm$1.3 \\
& P@3 & \textbf{36.65}$\pm$0.95 & 28.49$\pm$0.73 \\
& P@5 & \textbf{21.99}$\pm$0.57 & 20.67$\pm$0.67 \\
\midrule
\multirow{3}{*}{\textbf{Delicious}} 
& P@1	& \textbf{97.36}$\pm$0.37 & 61.78$\pm$0.91 \\
& P@3	& \textbf{69.40}$\pm$0.98 & 56.24$\pm$0.84 \\
& P@5	& 45.07$\pm$0.93 & \textbf{51.46}$\pm$0.84 \\
\midrule
\multirow{3}{*}{\textbf{Mediamill}} 
& P@1	& \textbf{93.57}$\pm$0.35 & 77.14$\pm$0.21 \\
& P@3	& \textbf{71.81}$\pm$1.23 & 58.64$\pm$0.32 \\
& P@5	& \textbf{46.55}$\pm$0.97 & \textbf{46.12}$\pm$0.11 \\
\midrule
\multirow{3}{*}{\textbf{Eurlex}} 
& P@1	& \textbf{83.18}$\pm$0.97 & 54.93$\pm$6.06 \\
& P@3	& \textbf{46.90}$\pm$2.89 & 41.50$\pm$4.89 \\
& P@5	& 28.56$\pm$1.88 & \textbf{33.61}$\pm$4.14 \\
\midrule
%\multirow{3}{*}{\textbf{Eurlex-4.3K}} 
%& P@1	& \textbf{85.99}$\pm$0.39 & --- \\
%& P@3	& \textbf{72.23}$\pm$2.19 & --- \\
%& P@5	& \textbf{48.04}$\pm$2.18 & --- \\
%\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} 
& P@1	& 74.16$\pm$2.37 & \textbf{76.03} \\
& P@3	& 27.88$\pm$0.29 & \textbf{64.63} \\
& P@5	& 16.75$\pm$0.18 & \textbf{56.60} \\
\bottomrule
\end{tabular} \caption{Mean and standard deviations precision@k over 10 different publicly-available train/validation splits.}\label{tab:baseline_seq2seq_precisions_no_propensity}
\end{table} 

==> ensemble_table_nDCG.tex <==
\begin{table}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lcccc }
\toprule
&& \textbf{Proposed} & \textbf{SLEEC} &	\textbf{FastXML}	 \\
\midrule
\multirow{3}{*}{\textbf{Bibtex}} & 
nDCG@1	 & \textit{64.56} & \textbf{65.08} & 63.42 \\ &
nDCG@3   & \textit{60.11} & \textbf{60.47} & 59.51 \\ &
nDCG@5	 & \textit{62.18} & \textbf{62.64} & 61.70 \\ 
\midrule
\multirow{3}{*}{\textbf{Delicious}} & 
nDCG@1	& 65.13 & 67.59 & \textbf{69.61}\\ &
nDCG@3	& 60.51 & 62.87 & \textbf{65.47}\\ &
nDCG@5	& 57.12 & 59.28 & \textbf{61.90} \\ 
\midrule
\multirow{3}{*}{\textbf{Mediamill}} & 
nDCG@1	 &  84.25 & \textbf{87.82} & 84.22 \\ &
nDCG@3	 &  75.33 & \textbf{81.50} & 75.41 \\ &
nDCG@5	 &  72.03 & \textbf{79.22} & 72.37 \\ 
\midrule
\multirow{3}{*}{\textbf{Eurlex}} & 
nDCG@1	 & \textbf{81.04} & 79.26 & 71.36 \\ &
nDCG@3	 & \textbf{71.29} & 68.13 & 62.87 \\ &
nDCG@5	 & \textbf{65.64} & 61.60 & 58.06 \\ 
\midrule
\multirow{3}{*}{\textbf{Wiki10}} & 
nDCG@1	& \textbf{86.05} & 85.88 & 84.31 \\ &
nDCG@3	& \textbf{79.11} & 72.98 & 75.35 \\ &
nDCG@5	& \textbf{72.26} & 62.70 & 63.36 \\  
\bottomrule
\end{tabular} \caption{nDCG@k on the ensemble-based nonlinear models. Best in \textbf{bold} and not significantly different to best in \textit{italics}.}\label{tbl_ensemble_d1}

\end{table} 

==> ensemble_table_p.tex <==
\begin{table}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lcccc }
\toprule
&& \textbf{Proposed} & \textbf{SLEEC} &	\textbf{FastXML}	 \\
\midrule
\multirow{3}{*}{\textbf{Bibtex}} & P@1 & \textit{64.56}$\pm$0.79 & \textbf{65.08}$\pm$0.65 &  63.42$\pm$0.67\\
& P@3 & \textit{39.51}$\pm$0.34 & \textbf{39.64}$\pm$0.39 &  39.23$\pm$0.57\\
& P@5 & \textit{28.80}$\pm$0.26 & \textbf{28.87}$\pm$0.32&  28.86$\pm$0.38\\

\midrule
\multirow{3}{*}{\textbf{Delicious}} & P@1 & 65.13$\pm$0.39 & 67.59$\pm$0.53 & \textbf{69.61}$\pm$0.58 \\
& P@3 & 59.07$\pm$0.41 & 61.38$\pm$0.59 & \textbf{64.12}$\pm$0.75 \\
& P@5	& 54.52$\pm$0.34 & 56.56$\pm$0.54 & \textbf{59.27}$\pm$0.65 \\

\midrule
\multirow{3}{*}{\textbf{Mediamill}} & P@1	& 84.25$\pm$0.27 & \textbf{87.82}$\pm$0.33 & 84.22$\pm$0.27 \\
& P@3	& 67.29$\pm$0.24 & \textbf{73.45}$\pm$0.30 & 67.33$\pm$0.20 \\
& P@5	& 52.90$\pm$0.15 & \textbf{59.17}$\pm$0.34 & 53.04$\pm$0.18 \\

\midrule
\multirow{3}{*}{\textbf{Eurlex}} & P@1	& \textbf{81.04}$\pm$0.81 & 79.26$\pm$0.86 & 71.36$\pm$1.63 \\
& P@3	& \textbf{67.91}$\pm$0.97 & 64.30$\pm$0.88 & 59.90$\pm$1.58 \\
& P@5	& \textbf{56.81}$\pm$0.97 & 52.33$\pm$0.80 & 50.39$\pm$1.40 \\

\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} & P@1	& \textbf{86.05} & 85.88 &  83.03\\
& P@3	& \textbf{76.85} & 72.98 &  67.47\\
& P@5	& \textbf{67.77} & 62.70 &  57.76\\
\bottomrule
\end{tabular}  \caption{Validation precision@k for ensemble-based non-linear models. Best in \textbf{bold} and not significantly different to best in \textit{italics}.}\label{tbl_ensemble_p1} 

\end{table}

==> modified_table_1.tex <==
\begingroup
\setlength{\tabcolsep}{5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.0} % Default
\begin{table*}[!htb]
\scriptsize 
\centering
\begin{tabular}{ lccccccc cccccc }
\toprule
&& \multicolumn{2}{c}{\textbf{Proposed}} & \multicolumn{2}{c}{\textbf{PD-sparse}} &	\multicolumn{2}{c}{\textbf{LEML}} &	\multicolumn{2}{c}{\textbf{CPLST}} &	\multicolumn{2}{c}{\textbf{CS}} &	\multicolumn{2}{c}{\textbf{ML-CSSP}} \\
\midrule
&  & \textbf{P} & \textbf{nDCG} & \textbf{P} & \textbf{nDCG} &	\textbf{P} & \textbf{nDCG} &	\textbf{P} & \textbf{nDCG} &	\textbf{P} & \textbf{nDCG} &	\textbf{P} & \textbf{nDCG} \\
\midrule
\multirow{3}{*}{\textbf{Bibtex}} & \textbf{@1}	&  \textbf{64.56}  & \red{00.0} & 61.29  & \red{00.0} & 62.54 & \red{00.0} & 62.38 & \red{00.0} & 58.87 & \red{00.0} & 44.98 &  \red{00.0}  \\
& \textbf{@3} &  \textbf{39.51}  & \red{00.0} & 35.82  & \red{00.0} & 38.41 & \red{00.0} & 37.84 & \red{00.0} & 33.53 & \red{00.0} & 30.43 &  \red{00.0}  \\
& \textbf{@5}	& \textbf{28.80}  & \red{00.0} & 25.74 & \red{00.0} & 28.21 & \red{00.0} & 27.62 & \red{00.0} & 23.72 & \red{00.0} & 23.53 &  \red{00.0}    \\
%\midrule
%\multicolumn{7}{c}{Delicious}	\\
\midrule
\multirow{3}{*}{\textbf{Delicious}} & \textbf{@1}	& \textbf{65.13} & \red{00.0} & 51.82  & \red{00.0} & \textbf{65.67} & \red{00.0} & \textbf{65.31} & \red{00.0} & 61.36 & \red{00.0} & 63.04 &  \red{00.0}  \\
& \textbf{@3}	&  59.07 & \red{00.0} & 44.18  & \red{00.0} & \textbf{60.55} & \red{00.0} & 59.95 & \red{00.0} & 56.46 & \red{00.0} & 56.26 &  \red{00.0}  \\
& \textbf{@5}	& 54.52 & \red{00.0} & 38.95  & \red{00.0} & \textbf{56.08} & \red{00.0} & 55.31 & \red{00.0} & 52.07 & \red{00.0} & 50.16 & \red{00.0}   \\
\midrule
\multirow{3}{*}{\textbf{Mediamill}} & \textbf{@1}	& \textbf{84.25} & \red{00.0} & 81.86  & \red{00.0} & \textbf{84.01} & \red{00.0} & 83.35 & \red{00.0} & \textbf{83.82} & \red{00.0} & 78.95 &  \red{00.0}  \\
& \textbf{@3}	&  \textbf{67.29} & \red{00.0} & 62.52  & \red{00.0} & \textbf{67.20} & \red{00.0} & 66.18 & \red{00.0} & \textbf{67.32} & \red{00.0} & 60.93 &  \red{00.0}  \\
& \textbf{@5}	 & \textbf{52.90} & \red{00.0}  & 45.11 & \red{00.0} & 52.80 & \red{00.0} & 51.46 & \red{00.0} & 52.80 & \red{00.0} & 44.27 &  \red{00.0}  \\
%\midrule
%\multicolumn{7}{c}{Eurlex} \\
\midrule
\multirow{3}{*}{\textbf{Eurlex}}  & \textbf{@1}	& \textbf{81.04} & \red{00.0} & 76.43  & \red{00.0} & 63.40 & \red{00.0} & 72.28 & \red{00.0} & 58.52 & \red{00.0} & 62.09 &  \red{00.0}  \\
& \textbf{@3}	& \textbf{67.91} & \red{00.0} & 60.37 & \red{00.0} & 50.35 & \red{00.0} & 58.16 & \red{00.0} & 45.51 & \red{00.0} & 48.39 &  \red{00.0}  \\
& \textbf{@5}	& \textbf{56.81} & \red{00.0} & 49.72 & \red{00.0} & 41.28 & \red{00.0} & 47.73 & \red{00.0} & 32.47 & \red{00.0} & 40.11 & \red{00.0}  \\
%\midrule
%\multicolumn{7}{c}{Wiki10-31k}	\\
\midrule
\multirow{3}{*}{\textbf{Wiki10-31k}} & \textbf{@1}	& \textbf{86.05} & \red{00.0} & 82.14 & \red{00.0} & 73.47 & \red{00.0} & -- & -- & -- & -- & -- &  -- \\
& \textbf{@3}	& \textbf{76.85} & \red{00.0} & 69.68 & \red{00.0} & 62.43 & \red{00.0} & -- & -- & -- & -- & -- & --  \\
& \textbf{@5}	& \textbf{67.77} & \red{00.0} & 58.76 & \red{00.0} & 54.35 & \red{00.0} & -- & -- & -- & -- & -- &  -- \\
\bottomrule
\end{tabular} \caption{Validation set top-$k$ label precision (P@k) and normalised Discounted Cumulative Gain (nDCG@k). We show means over 10 runs with single models and $k=100$ or $30$ (Mediamill). Best model(s) per metric highlighted in \textbf{bold} ($p=0.05$). In supplementary material we additionally report all models' variances.}\label{tbl_smallp1_m}
\end{table*} 
\endgroup
